Enhancing Temporal Consistency in Video Editing by Reconstructing Videos with 3D Gaussian Splatting

Recent advancements in zero-shot video diffusion models have shown promise for text-driven video editing, but challenges remain in achieving high temporal consistency. To address this, we introduce Video-3DGS, a 3D Gaussian Splatting (3DGS)-based video refiner designed to enhance temporal consistency in zero-shot video editors. Our approach utilizes a two-stage 3D Gaussian optimizing process tailored for editing dynamic monocular videos. In the first stage, Video-3DGS employs an improved version of COLMAP, referred to as MC-COLMAP, which processes original videos using a Masked and Clipped approach. For each video clip, MC-COLMAP generates the point clouds for dynamic foreground objects and complex backgrounds. These point clouds are utilized to initialize two sets of 3D Gaussians (Frg-3DGS and Bkg-3DGS) aiming to represent foreground and background views. Both foreground and background views are then merged with a 2D learnable parameter map to reconstruct full views. In the second stage, we leverage the reconstruction ability developed in the first stage to impose the temporal constraints on the video diffusion model. To demonstrate the efficacy of Video-3DGS on both stages, we conduct extensive experiments across two related tasks: Video Reconstruction and Video Editing. Video-3DGS trained with 3k iterations significantly improves video reconstruction quality (+3 PSNR, +7 PSNR increase) and training efficiency (x1.9, x4.5 times faster) over NeRF-based and 3DGS-based state-of-art methods on DAVIS dataset, respectively. Moreover, it enhances video editing by ensuring temporal consistency across 58 dynamic monocular videos.

==> sections/2.related.tex <==
\section{Related Work}
\inkyu{We can move Related work part to Appendix so that it can save more space for much important contents.}
\label{sec:related}


{\bf Video Representation}

{\bf Video Reconstruction}

{\bf Video Editing}

==> table/edit_table.tex <==

% LPIPS↓ 
% CoDeF & {31.26} & 0.9254 & 0.0735 & 29.11 & 0.9451 & 0.0601 \\
% RobustDyn & 24.58 & 0.9520 & 0.0824 & 32.50 & 0.9713 & 0.0362 \\
% Ours & {41.54} & {0.9873} & {0.0234} & {42.63} & 0.9951 & {0.0052} \\
\begin{table*}
\centering
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{l|l||cc|cc||cc|cc||cc|cc}
\toprule
\toprule
% & \multicolumn{2}{c}{bear} & \multicolumn{2}{2}{car-shadow} & \multicolumn{2}{c}{dog} & \multicolumn{2}{c}{elephant} & \multicolumn{2}{c}{gold-fish} & \multicolumn{2}{c}{hike} & \multicolumn{2}{c}{horsejump-low} \\
\multirow{2}{*}{Prompt} & \multirow{2}{*}{\diagbox{Dataset}{Method}} & \multicolumn{2}{c}{Text2Vid-Zero} & \multicolumn{2}{c||}{+\modelname} & \multicolumn{2}{c}{TokenFlow} & \multicolumn{2}{c||}{+\modelname} & \multicolumn{2}{c}{RAVE} & \multicolumn{2}{c}{+\modelname} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15}
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14} 
 & & WarpSSIM↑ & $Q_{edit}$↑ &  WarpSSIM↑ & $Q_{edit}$↑ &  WarpSSIM↑ & $Q_{edit}$↑ &  WarpSSIM↑ & $Q_{edit}$↑ &  WarpSSIM↑ & $Q_{edit}$↑ &  WarpSSIM↑ & $Q_{edit}$↑  \\

\midrule
\multirow{3}{*}{Style change} & DAVIS & {0.729} & {21.1} & {0.841} (\textcolor{blue}{+11.2\%}) & {22.8} (\textcolor{blue}{+1.7\%}) & {0.869} & {23.2} & {0.916} (\textcolor{blue}{+4.7\%}) & {24.4} (\textcolor{blue}{+1.2\%})  & {0.874} & {24.8} & {0.905} (\textcolor{blue}{+3.1\%}) & {25.6} (\textcolor{blue}{+0.8\%}) \\

& Videovo & {0.771} & {21.7} & {0.908} (\textcolor{blue}{+13.7\%}) & {22.9} (\textcolor{blue}{+1.7\%}) & {0.900} & {22.8} & {0.934} (\textcolor{blue}{+3.4\%}) & {24.2} (\textcolor{blue}{+1.4\%}) & {0.879} & {21.8} & {0.920} (\textcolor{blue}{+4.1\%}) & {23.7} (\textcolor{blue}{+1.9\%}) \\

& Youtube & 0.739 & 21.5 & {0.899} (\textcolor{blue}{+16.0\%}) & {21.9} (\textcolor{blue}{+0.4\%}) & 0.855 & 22.1 & {0.926} (\textcolor{blue}{+7.1\%}) & {24.2} (\textcolor{blue}{+2.1\%}) & 0.848 & 22.6 & {0.916} (\textcolor{blue}{+6.8\%}) & {24.1} (\textcolor{blue}{+1.5\%}) \\

\midrule
\multirow{3}{*}{Object change} & DAVIS & {0.682} & {19.0} & {0.820} (\textcolor{blue}{+13.8\%}) & {19.9} (\textcolor{blue}{+0.9\%}) & {0.853}  & {22.1} & {0.909} (\textcolor{blue}{+5.6\%}) & {22.9} (\textcolor{blue}{+0.8\%}) & {0.877}  & {23.7} & {0.908} (\textcolor{blue}{+3.1\%}) & {23.7}(+0.0\%)   \\

& Videovo & {0.814} & {22.8} & {0.917} (\textcolor{blue}{+10.3\%}) & {21.3} (\textcolor{red}{-1.5\%}) & {0.891}  & {22.6} & {0.931} (\textcolor{blue}{+4.0\%}) & {22.9} (\textcolor{blue}{+0.3\%}) & {0.875}  & {22.3} & {0.916} (\textcolor{blue}{+4.1\%}) & {23.1} (\textcolor{blue}{+0.8\%})  \\

& Youtube & 0.702 & 19.2 & {0.884} (\textcolor{blue}{+18.2\%}) & {19.2} (\textcolor{black}{+0.0\%}) &0.831 & 21.7 & {0.926} (\textcolor{blue}{+9.5\%}) & {22.9} (\textcolor{blue}{+1.2\%}) & 0.848 & 21.1 & {0.916} (\textcolor{blue}{+6.8\%}) & {22.7} (\textcolor{blue}{+1.6\%})\\

\midrule
\multirow{3}{*}{Background change} & DAVIS & {0.674} & {19.0} & {0.823} (\textcolor{blue}{+14.9\%}) & {20.1} (\textcolor{blue}{+1.1\%}) & {0.855} & {23.4} & {0.908} (\textcolor{blue}{+5.3\%}) & {24.5} (\textcolor{blue}{+1.1\%}) & {0.859}  & {22.8} & {0.901} (\textcolor{blue}{+4.2\%}) & {23.3} (\textcolor{blue}{+0.5\%}) \\

& Videovo & {0.737} & {21.0} & {0.885} (\textcolor{blue}{+14.8\%}) & {21.9} (\textcolor{blue}{+0.9\%}) & {0.906} & {23.5} & {0.937} (\textcolor{blue}{+3.1\%}) & {24.2} (\textcolor{blue}{+0.7\%}) & {0.861}  & {24.3} & {0.901} (\textcolor{blue}{+4.0\%}) & {24.7} (\textcolor{blue}{+0.4\%})  \\

& Youtube & 0.689 & 19.6 & {0.888} (\textcolor{blue}{+19.9\%}) & {20.5} (\textcolor{blue}{+0.9\%}) & 0.846 & 22.0 & {0.917} (\textcolor{blue}{+7.1\%}) & {22.9} (\textcolor{blue}{+0.9\%}) & 0.859 & 21.3 & {0.918} (\textcolor{blue}{+5.9\%}) & {22.4} (\textcolor{blue}{+1.1\%}) \\


\midrule
\multirow{3}{*}{Multiple change} & DAVIS & {0.678} & {21.1} & {0.823} (\textcolor{blue}{+14.5\%}) & {21.3} (\textcolor{blue}{+0.2\%}) & {0.842} & {23.0} & {0.903} (\textcolor{blue}{+6.1\%}) & {23.7} (\textcolor{blue}{+0.7\%}) & {0.879}  & {22.1} & {0.918} (\textcolor{blue}{+3.9\%}) & {23.7} (\textcolor{blue}{+1.6\%}) \\

& Videovo &{0.770} & {21.9} & {0.896} (\textcolor{blue}{+12.6\%}) & {22.2} (\textcolor{blue}{+0.3\%}) & {0.890} & {21.3} & {0.929} (\textcolor{blue}{+3.9\%}) & {22.5} (\textcolor{blue}{+1.2\%}) & {0.871}  & {21.1} & {0.913} (\textcolor{blue}{+4.2\%}) & {22.4} (\textcolor{blue}{+1.3\%}) \\

& Youtube & 0.675 & 19.0 & {0.870} (\textcolor{blue}{+19.5\%}) & {19.9} (\textcolor{blue}{+0.9\%}) & 0.860 & {22.4}& {0.921} (\textcolor{blue}{+6.1\%})& 22.3 (\textcolor{red}{-0.1\%}) & 0.865 & 21.8 & 0.920 (\textcolor{blue}{+5.5\%}) & 22.2 (\textcolor{blue}{+0.4\%}) \\

\bottomrule
% \bottomrule
\rowcolor{lightgray}
\multicolumn{2}{c||}{Average} & 0.722 & 20.6 & 0.871 (\textcolor{blue}{+14.9\%}) & 21.2 (\textcolor{blue}{+0.6\%}) & 0.867 & 22.5 & 0.921 (\textcolor{blue}{+5.4\%}) & 23.5 (\textcolor{blue}{+1.0\%}) & 0.866 & 22.5  & 0.913 (\textcolor{blue}{+4.7\%}) & 23.5 (\textcolor{blue}{+1.0\%}) \\

\bottomrule
\bottomrule
\end{tabular}
}
\vspace{-2mm}
\caption{Quantitative results  of Video Editing on three different datasets: DAVIS, Videvo, Youtube. We present the results for WarpSSIM and $Q_{edit}$,
with text color indicating the effect of \modelname.
Across almost all settings, our \modelname increases both temporal consistency and overall video editing performance.
↑: the higher, the better.
}
\label{tab:edit_quan}
\end{table*}

==> table/edit_table_w_fatezero.tex <==

% LPIPS↓ 
% CoDeF & {31.26} & 0.9254 & 0.0735 & 29.11 & 0.9451 & 0.0601 \\
% RobustDyn & 24.58 & 0.9520 & 0.0824 & 32.50 & 0.9713 & 0.0362 \\
% Ours & {41.54} & {0.9873} & {0.0234} & {42.63} & 0.9951 & {0.0052} \\
\begin{table*}
\centering
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{l|l||cc|cc||cc|cc||cc|cc||cc|cc}
\toprule
% & \multicolumn{2}{c}{bear} & \multicolumn{2}{2}{car-shadow} & \multicolumn{2}{c}{dog} & \multicolumn{2}{c}{elephant} & \multicolumn{2}{c}{gold-fish} & \multicolumn{2}{c}{hike} & \multicolumn{2}{c}{horsejump-low} \\
\multirow{2}{*}{Prompt} & \multirow{2}{*}{\diagbox{Dataset}{Method}} & \multicolumn{2}{c}{Text2Vid-Zero} & \multicolumn{2}{c||}{+Video-3DGS-Edit} & \multicolumn{2}{c}{TokenFlow} & \multicolumn{2}{c||}{+Video-3DGS-Edit} & \multicolumn{2}{c}{RAVE} & \multicolumn{2}{c||}{+Video-3DGS-Edit} & \multicolumn{2}{c}{FateZero} & \multicolumn{2}{c}{+Video-3DGS-Edit}   \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15}
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} \cmidrule(lr){11-12} \cmidrule(lr){13-14} \cmidrule(lr){15-16} \cmidrule(lr){17-18}
 & & WarpSSIM↑ & $Q_{edit}$↑ &  WarpSSIM↑ & $Q_{edit}$↑ &  WarpSSIM↑ & $Q_{edit}$↑ &  WarpSSIM↑ & $Q_{edit}$↑ &  WarpSSIM↑ & $Q_{edit}$↑ &  WarpSSIM↑ & $Q_{edit}$↑ &  WarpSSIM↑ & $Q_{edit}$↑ &  WarpSSIM↑ & $Q_{edit}$↑ \\

\midrule
\multirow{3}{*}{Style change} & DAVIS & {0.729} & {21.1} & {0.841} (\textcolor{blue}{+0.112}) & {22.8} (\textcolor{blue}{+1.7}) & {0.869} & {23.2} & {0.916}(\textcolor{blue}{+0.05}) & {24.4}(\textcolor{blue}{+1.2})  & {0.874} & {24.8} & {0.905} & {25.6} &  {0.918} & {22.1} & {0.939} & {22.3} \\

& Videovo & {0.771} & {21.7} & {0.908} & {22.9} & {0.900} & {22.8} & {0.934} & {24.2} & {0.879} & {21.8} & {0.920} & {23.7} & {0.912} & {22.5} & {0.933} & {23.2} \\

& Youtube & 0.739 & 21.5 & {0.899} & {21.9}  & 0.855 & 22.1 & {0.926} & {24.2} & 0.848 & 22.6 & {0.916} & {24.1} \\

\midrule
\multirow{3}{*}{Object change} & DAVIS & {0.682} & {19.0} & {0.820} & {19.9} & {0.853}  & {22.1} & {0.909} & {22.9} & {0.877}  & {23.7} & {0.908} & {23.7} & 0.916 & {21.6} & {0.938} & {21.6} \\

& Videovo & {0.814} & {22.8} & {0.917} & {21.3} & {0.891}  & {22.6} & {0.931} & {22.9} & {0.875}  & {22.3} & {0.916} & {23.1}  & 0.901 & 21.6 & {0.929} & {22.0} \\

& Youtube & 0.702 & 19.2 & {0.884} & {19.2} &0.831 & 21.7 & {0.926} & {22.9} & 0.848 & 21.1 & {0.916} & {22.7}\\

\midrule
\multirow{3}{*}{Background change} & DAVIS & {0.674} & {19.0} & {0.823} & {20.1} & {0.855} & {23.4} & {0.908} & {24.5} & {0.859}  & {22.8} & {0.901} & {23.3} & 0.909 & 20.6 & {0.935} & {20.8}\\

& Videovo & {0.737} & {21.0} & {0.885} & {21.9} & {0.906} & {23.5} & {0.937} & {24.2} & {0.861}  & {24.3} & {0.901} & {24.7} & 0.911 & 22.3 & {0.933} & {22.9} \\

& Youtube & 0.689 & 19.6 & {0.888} & {20.5} & 0.846 & 22.0 & {0.917} & {22.9} & 0.859 & 21.3 & {0.918} & {22.4} \\


\midrule
\multirow{3}{*}{Multiple change} & DAVIS & {0.678} & {21.1} & {0.823} & {21.3} & {0.842} & {23.0} & {0.903} & {23.7} & {0.879}  & {22.1} & {0.918} & {23.7} & 0.908 & {19.3} & {0.934} & 19.0 \\

& Videovo &{0.770} & {21.9} & {0.896} & {22.2} & {0.890} & {21.3} & {0.929} & {22.5} & {0.871}  & {21.1} & {0.913} & {22.4} & 0.904& 20.9 & {0.929} & {21.3}\\

& Youtube & 0.675 & 19.0 & {0.870} & {19.9} & 0.860 & {22.4}& {0.921}& 22.3 & 0.865 & 21.8 & 0.920 & 22.2 \\

\bottomrule

\end{tabular}
}
\caption{Quantitative results (WarpSSIM/$Q_{edit}$)  of Video Editing on three different datasets DAVIS, Videvo, Youtube. We present the results for WarpSSIM and $Q_{edit}$,
with text color indicating the effect of \modelname. It proves that our Video-3DGS-Edit mostly increase both temporal consistency while maintaining overall video editing performance.
}
\label{tab:edit_quan}
\end{table*}

==> table/progressive_edit.tex <==
\begin{table*}
\centering
\resizebox{0.9\linewidth}{!}{
\begin{tabular}{cl|cc||c|cc||c|cc}
\hline
 \multicolumn{2}{c|}{Text2Video-Zero}             & \multicolumn{2}{c||}{+Video-3DGS}                                                          & TokenFlow                   & \multicolumn{2}{c||}{+Video-3DGS}                                                        & RAVE                        & \multicolumn{2}{c}{+Video-3DGS}                                                         \\ \hline
 \multicolumn{2}{c|}{WarpSSIM / Qedit} & & WarpSSIM / Qedit & WarpSSIM / Qedit & & WarpSSIM / Qedit & WarpSSIM / Qedit & & WarpSSIM / Qedit \\
  \hline
\multicolumn{2}{c|}{\multirow{2}{*}{0.729 / 21.1}} & \begin{tabular}[c]{@{}c@{}}Single update \end{tabular} & 0.841 / 22.8 & \multirow{2}{*}{0.869/23.2} & \begin{tabular}[c]{@{}c@{}}Single update \end{tabular} & 0.916 / 24.4 & \multirow{2}{*}{0.874 / 24.8} & \begin{tabular}[c]{@{}c@{}}Single update \end{tabular} & 0.905 / 25.6 \\ \cline{3-4} \cline{6-7} \cline{9-10} 
\multicolumn{2}{c|}{}                            & \begin{tabular}[c]{@{}c@{}}Progressive update \end{tabular}   & 0.872 / 24.2  &                  & \begin{tabular}[c]{@{}c@{}}Progressive update \end{tabular}   & 0.922 / 25.4 &                             & \begin{tabular}[c]{@{}c@{}}Progressive update 
\end{tabular}   & 0.908 / 26.5  \\ \hline
\end{tabular}
}
\caption{{Performance relationship between video reconstruction and video editing (`style change' in DAVIS).}
}
\label{tab:progressive}
\end{table*}

==> table/qual_fig.tex <==
\begin{figure*}[t]
    \centering 
    \includegraphics[width=0.93\textwidth]{icml2024/figures/qual_figure.pdf}
    \caption{\textbf{Qualitative comparison with the baselines for video reconstruction and video editing} 
    }
    \label{fig:qualitative}
    % \vspace{-3mm}
\end{figure*}

==> table/recon_bilateral.tex <==
\begin{table}
\centering

\resizebox{0.9\linewidth}{!}{
\begin{tabular}{|c|cc|cc|}
\hline
\multirow{2}{*}{\diagbox{Dataset}{Method}} & \multicolumn{2}{c|}{wo/ TF loss} & \multicolumn{2}{c|}{w/ TF loss} \\
\cline{2-5}
 & PSNR & SSIM & PSNR & SSIM \\
\hline
DAVIS & & & & \\
\hline
\end{tabular}
}
\caption{Ablation study on TF(texture-focused) loss}
\label{tab:TF}
\end{table}


==> table/recon_dualsingle.tex <==
\begin{table}
\centering

\resizebox{0.9\linewidth}{!}{
\begin{tabular}{|c|cc|cc|}
\hline
\multirow{2}{*}{\diagbox{Dataset}{Method}} & \multicolumn{2}{c|}{Dual-branch} & \multicolumn{2}{c|}{Single-branch} \\
\cline{2-5}
 & PSNR & SSIM & PSNR & SSIM \\
\hline
DAVIS & & & & \\
\hline
\end{tabular}
}
\caption{Dual-branch vs. Single-branch}
\label{tab:branch}
\end{table}


==> table/recon_group.tex <==
\begin{table}
\centering
\resizebox{1.1\linewidth}{!}{
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{\diagbox{Dataset}{Group size}} & \multicolumn{2}{c|}{1} & \multicolumn{2}{c|}{2} & \multicolumn{2}{c|}{4} & \multicolumn{2}{c|}{All} \\
\cline{2-9}
 & PSNR & Time & PSNR & Time & PSNR & Time & PSNR & Time  \\
\hline
DAVIS & 37.3 & 12m & 33.3 & 6m & 30.2 & 4m  & 27.5 & 2m \\
\hline
\end{tabular}
}
\caption{iteration 3k}
\label{tab:group}
\end{table}

\begin{table}
\centering
\resizebox{1.1\linewidth}{!}{
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{\diagbox{Dataset}{Group size}} & \multicolumn{2}{c|}{1} & \multicolumn{2}{c|}{2} & \multicolumn{2}{c|}{4} & \multicolumn{2}{c|}{All} \\
\cline{2-9}
 & PSNR & Time & PSNR & Time & PSNR & Time & PSNR & Time  \\
\hline
DAVIS & 41.2 & 22m & 36.1 & 11m & 32.4 & 7m & 29.7 & 4m \\
\hline
\end{tabular}
}
\caption{iteration 5k}
\label{tab:group}
\end{table}

\begin{table}
\centering
\resizebox{1.1\linewidth}{!}{
\begin{tabular}{|c|cc|cc|cc|cc|}
\hline
\multirow{2}{*}{\diagbox{Dataset}{Group size}} & \multicolumn{2}{c|}{1} & \multicolumn{2}{c|}{2} & \multicolumn{2}{c|}{4} & \multicolumn{2}{c|}{All} \\
\cline{2-9}
 & PSNR & Time & PSNR & Time & PSNR & Time & PSNR & Time  \\
\hline
DAVIS & 45.7 & 54m & 39.9 & 29m & 35.4 & 16m & 32.0 & 7m \\
\hline
\end{tabular}
}
\caption{iteration 3k}
\label{tab:group}
\end{table}




==> table/recon_singlemultideform.tex <==
\begin{table}
\centering

\resizebox{0.9\linewidth}{!}{
\begin{tabular}{|c|cc|cc|}
\hline
\multirow{2}{*}{\diagbox{Dataset}{Method}} & \multicolumn{2}{c|}{Multi-deform} & \multicolumn{2}{c|}{Single-deform} \\
\cline{2-5}
 & PSNR & SSIM & PSNR & SSIM \\
\hline
DAVIS & & & & \\
\hline
\end{tabular}}
\caption{Multiple-deform vs. Single-deform}
\label{tab:deformnumber}
\end{table}


==> table/recon_table.tex <==

% LPIPS↓ 
% CoDeF~\cite{ouyang2023codef} & \graycell{31.26} & 0.9254 & 0.0735 & 29.11 & 0.9451 & 0.0601 \\
% Robust-Dyn~\cite{liu2023robust} & 24.58 & 0.9520 & 0.0824 & 32.50 & 0.9713 & 0.0362 \\
% Ours & \redcell{41.54} & \redcell{0.9873} & \redcell{0.0234} & \redcell{42.63} & 0.9951 & \redcell{0.0052} \\
\begin{table*}
\centering
\resizebox{0.95\linewidth}{!}{
\begin{tabular}{lccccccccccccccccccccc}
\toprule
\toprule
% & \multicolumn{2}{c}{bear} & \multicolumn{2}{2}{car-shadow} & \multicolumn{2}{c}{dog} & \multicolumn{2}{c}{elePhant} & \multicolumn{2}{c}{gold-fish} & \multicolumn{2}{c}{hike} & \multicolumn{2}{c}{horsejumP-low} \\
\multirow{2}{*}{\diagbox{Method}{Scene}} & \multicolumn{3}{c}{bear} & \multicolumn{3}{c}{car-shadow} & \multicolumn{3}{c}{dog} & \multicolumn{3}{c}{elephant} & \multicolumn{3}{c}{gold-fish} & \multicolumn{3}{c}{hike} & \multicolumn{3}{c}{horsejump-low} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15}
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22}
 & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓  & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓\\

\midrule
Robust-Dyn~\cite{liu2023robust} & 27.2 & 0.785 & 840m & 31.6 & 0.944  & 660m & 27.5 & 0.777 & 780m & 28.6 & 0.823 & 840m & 28.5 & 0.842 & 840m & 27.3 & 0.882 & 780m & 24.9 & 0.667 & 720m\\
NLA~\cite{kasten2021layered} & 26.7 & 0.798 & 323m & 30.7 & 0.913 & 307m & 27.5 & 0.732 & 325m & 26.5 & 0.758 & 295m & 28.5 & 0.879 & 306m & 24.0 & 0.686 & 304m & 25.6 & 0.737 & 315m
\\
CoDeF~\cite{ouyang2023codef} & 28.5 & 0.851  & \graycell{27m}  & 31.0 & 0.917 & \graycell{18m} & 31.7 & 0.906 & \graycell{22m} & 30.6 & 0.882 & \graycell{28m} & 30.9 & 0.895 & 28m & 27.0 & 0.808 & 28m & 28.0 & 0.824 & \graycell{29m}  \\
\hline
% 3DGS$\ast$~\cite{kerbl20233d} &  &  &  &  &  &  \\
% Deform-3DGS$\ast$~\cite{yang2023deformable3dgs} &  &  &  &  &  &  \\
% 3DGS$\diamond$ &  &  &  &  &  &  \\
% Deform-3DGS$\diamond$ &  &  &  &  &  & &  &  &  \\
3DGS~\cite{kerbl20233d} & 29.1 & 0.927 & \redcell{7m} & \multicolumn{3}{c}{N/A} & 27.1 & 0.839 & \redcell{9m} & 31.2  & 0.928 & \redcell{8m} & 23.7 & 0.860 & \redcell{6m} & 19.3 & 0.436 & \yellowcell{14m} & \multicolumn{3}{c}{N/A}    \\
Deform-3DGS~\cite{yang2023deformable3dgs} & 33.1 & 0.954  & 46m & \multicolumn{3}{c}{N/A} & 32.4 & 0.916 & 53m  & 35.2 & 0.949 & 37m & 30.8 & 0.919 & \graycell{16m} &  27.3 & 0.880 & 72m  & \multicolumn{3}{c}{N/A} \\
\hline
\modelname (w/ \textit{3k} iterations) & \graycell{34.6} & \graycell{0.974} & \yellowcell{15m}  & \graycell{37.5} & \graycell{0.986} & \redcell{6m} & \graycell{40.0} & \graycell{0.984} & \yellowcell{10m} & \graycell{36.9} & \graycell{0.980} & \yellowcell{13m} & \graycell{43.1} & \graycell{0.982} & \yellowcell{12m} & \graycell{35.7} & \graycell{0.981} & \redcell{12m} &  \graycell{34.1} &  \graycell{0.970} & \redcell{10m} \\
\modelname (w/ \textit{5k} iterations) & \yellowcell{38.3} & \yellowcell{0.985} & 32m  & \yellowcell{42.7} & \yellowcell{0.993} & \yellowcell{11m} & \yellowcell{43.6} & \yellowcell{0.992} & 20m & \yellowcell{40.9} & \yellowcell{0.989} & 21m & \yellowcell{45.4} & \yellowcell{0.988} & 20m & \yellowcell{39.1} & \yellowcell{0.990} & \graycell{26m} & \yellowcell{36.9} & \yellowcell{0.979} & \yellowcell{20m} \\
\modelname (w/ \textit{10k} iterations) & \redcell{44.8} & \redcell{0.994}  & 97m & \redcell{47.7}  & \redcell{0.996}  & 27m  & \redcell{47.6} & \redcell{0.996} & 47m & \redcell{45.1} & \redcell{0.995} & 54m & \redcell{47.9} & \redcell{0.992} & 42m & \redcell{44.3} & \redcell{0.997} & 78m & \redcell{42.5} & \redcell{0.993} & 61m \\
\bottomrule
\bottomrule
% & \multicolumn{2}{c}{lab-coat} & \multicolumn{2}{c}{longboard} & \multicolumn{2}{c}{motorbike} & \multicolumn{2}{c}{swing} & \multicolumn{2}{c}{blackswan} & \multicolumn{2}{c}{camel} & \multicolumn{2}{c}{car-turn} \\
\multirow{2}{*}{\diagbox{Method}{Scene}} & \multicolumn{3}{c}{lab-coat} & \multicolumn{3}{c}{longboard} & \multicolumn{3}{c}{motorbike} & \multicolumn{3}{c}{swing} & \multicolumn{3}{c}{blackswan} & \multicolumn{3}{c}{camel} & \multicolumn{3}{c}{car-turn} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22}
& PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓  & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓\\
\midrule
Robust-Dyn~\cite{liu2023robust} & 25.7 & 0.783  & 720m  & 25.9  & 0.752 & 720m &  28.2 & 0.833 & 720m & 26.3 & 0.749 & 780m & 28.0 & 0.787 & 720m & 26.7 & 0.812 & 720m & 29.6 & 0.900 & 803m \\
NLA~\cite{kasten2021layered} & 27.5 & 0.732 & 308m  & 26.1 & 0.743 & 292m & 30.4 & 0.882 & 317m & 27.8 & 0.814 & 290m & 29.9 & 0.837 & 314m & 26.1 & 0.791 & 305m & 28.5 & 0.827 & 302m  \\
CoDeF~\cite{ouyang2023codef} & 31.6 & 0.910  & 28m  & 30.7  & 0.929 & 29m & 29.0 & 0.866 & 30m & 27.7 & 0.878 & \graycell{21m} & 29.5 & 0.867 & \graycell{28m} & 27.4 & 0.809 & \graycell{28m} & 28.9 & 0.830 & \yellowcell{28m} \\
\hline
3DGS~\cite{kerbl20233d} & 27.4 & 0.884 & \yellowcell{12m}  & 25.1 & 0.846 & \yellowcell{10m}  & 29.2 & 0.933 & \yellowcell{9m} & \multicolumn{3}{c}{N/A} & 25.1 & 0.832 & \redcell{8m} & \multicolumn{3}{c}{N/A} & \multicolumn{3}{c}{N/A} \\
Deform-3DGS~\cite{yang2023deformable3dgs} & 36.3 & 0.964 & 53m  & 31.4 & 0.928 & 54m & 36.9 & 0.969 & 45m & \multicolumn{3}{c}{N/A} & 28.0 & 0.843 & 52m & \multicolumn{3}{c}{N/A} & \multicolumn{3}{c}{N/A} \\
\hline
\modelname (w/ \textit{3k} iterations)  & \graycell{40.1} & \graycell{0.987} & \redcell{8m}  & \graycell{38.6} & \graycell{0.981} & \redcell{9m} & \graycell{38.6} & \graycell{0.983} & \redcell{8m} & \graycell{39.0} & \graycell{0.982} & \redcell{10m} & \graycell{38.1} & \graycell{0.981} & \redcell{8m} & \graycell{35.3} & \graycell{0.979} & \redcell{14m} & \graycell{33.1} & \graycell{0.964} & \redcell{15m}\\
\modelname (w/ \textit{5k} iterations) & \yellowcell{43.6} & \yellowcell{0.993} & \graycell{16m}  & \yellowcell{41.7}  & \yellowcell{0.990} & \graycell{18m} & \yellowcell{42.7} & \yellowcell{0.991} & \graycell{14m} & \yellowcell{42.8} & \yellowcell{0.991} & \yellowcell{18m} & \yellowcell{42.0} & \yellowcell{0.990} & \yellowcell{15m} & \yellowcell{38.8} & \yellowcell{0.988} & \yellowcell{26m} & \yellowcell{35.5} & \yellowcell{0.972} & \yellowcell{28m}\\
\modelname (w/ \textit{10k} iterations) & \redcell{47.8} &  \redcell{0.996} & 38m & \redcell{46.7} & \redcell{0.996}  & 45m & \redcell{46.4} & \redcell{0.995} & 34m & \redcell{46.3} & \redcell{0.995} & 44m & \redcell{45.3} & \redcell{0.996} & 34m & \redcell{44.2} & \redcell{0.995} & 74m & \redcell{39.4} & \redcell{0.982} & \graycell{76m} \\

\bottomrule
\bottomrule
% & \multicolumn{2}{c}{flamingo} & \multicolumn{2}{c}{hockey} & \multicolumn{2}{c}{kid-football} & \multicolumn{2}{c}{lucia} & \multicolumn{2}{c}{scooter-gray} & \multicolumn{2}{c}{boat} & \multicolumn{2}{c}{car-roundabout} \\
\multirow{2}{*}{\diagbox{Method}{Scene}} & \multicolumn{3}{c}{flamingo} & \multicolumn{3}{c}{hockey} & \multicolumn{3}{c}{kid-football} & \multicolumn{3}{c}{lucia} & \multicolumn{3}{c}{scooter-gray} & \multicolumn{3}{c}{boat} & \multicolumn{3}{c}{car-roundabout} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22}
 & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓  & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓\\
\midrule
Robust-Dyn~\cite{liu2023robust} & 26.5 & 0.728 & 780m  & 28.7 & 0.851  & 785m & 26.8 & 0.859 & 780m & 24.5 & 0.650 & 774m & 25.8 & 0.863 & 780m & 28.6 & 0.829 & 780m & 25.5 & 0.839 & 780m \\
NLA~\cite{kasten2021layered} & 28.2  & 0.800  & 321m  & 24.0 & 0.686  &  305m & 27.0 & 0.863 & 328m & 27.3 & 0.810 & 305m & 25.4 & 0.807 & 314m & 31.3 & 0.855 & 318m &  25.0 & 0.804 & 299m\\
CoDeF~\cite{ouyang2023codef} & 29.8 & 0.845 & 28m & 31.8 & 0.923  & 27m & 32.1 & 0.940 & 28m & 26.9 & 0.776 & 28m  & 26.4 & 0.863 & 33m & 33.2 & 0.900 & \graycell{28m} & 28.4 & 0.898 & 28m \\
\hline
3DGS~\cite{kerbl20233d}  & 23.8 & 0.830 & \redcell{7m} & 24.5 & 0.907 & \redcell{8m} & 20.9 & 0.864 & \yellowcell{12m} & \multicolumn{3}{c}{N/A} & 18.2 & 0.640 & \yellowcell{16m} & \multicolumn{3}{c}{N/A} & 22.5 & 0.867 & \redcell{10m}\\
Deform-3DGS~\cite{yang2023deformable3dgs} & 26.5  & 0.870 & 36m & 29.7 & 0.945 & 29m & 28.6 & 0.939 & 44m & \multicolumn{3}{c}{N/A} & 26.8 & 0.884 & 71m & \multicolumn{3}{c}{N/A} & 27.1 & 0.917 & 71m\\
\hline
\modelname (w/ \textit{3k} iterations) & \graycell{36.9} & \graycell{0.976} & \yellowcell{12m} & \graycell{39.3} & \graycell{0.982} & \yellowcell{13m} & \graycell{39.8} & \graycell{0.985} & \redcell{11m} & \graycell{34.1} & \graycell{0.963} & \redcell{11m} & \graycell{38.8} & \graycell{0.984} & \redcell{12m} & \graycell{40.5} & \graycell{0.984} & \redcell{8m} & \graycell{35.7} & \graycell{0.983} & \yellowcell{13m}\\
\modelname (w/ \textit{5k} iterations) & \yellowcell{40.9} & \yellowcell{0.987} & \graycell{22m} & \yellowcell{42.8} & \yellowcell{0.990} & \graycell{25m} & \yellowcell{42.6} & \yellowcell{0.990} & \graycell{21m} & \yellowcell{38.7} & \yellowcell{0.986} & \graycell{23m} & \yellowcell{43.4} & \yellowcell{0.993} & \graycell{24m} & \yellowcell{43.3} & \yellowcell{0.990} & \yellowcell{14m} & \yellowcell{40.8} & \yellowcell{0.993} & \graycell{25m} \\
\modelname (w/ \textit{10k} iterations) & \redcell{46.2} & \redcell{0.995} & 58m & \redcell{47.9} & \redcell{0.995} & 58m & \redcell{47.4} & \redcell{0.995} & 49m & \redcell{43.8} & \redcell{0.996} & 66m & \redcell{47.2} & \redcell{0.996} & 58m & \redcell{47.0} & \redcell{0.995} & 33m & \redcell{46.1} & \redcell{0.997} & 60m \\

\bottomrule
\bottomrule
% & \multicolumn{2}{c}{cows} & \multicolumn{2}{c}{drift-turn} & \multicolumn{2}{c}{horsejumP-high} & \multicolumn{2}{c}{kite-surf} & \multicolumn{2}{c}{mallard-water} & \multicolumn{2}{c}{mbike-trick} & \multicolumn{2}{c}{rhino} \\
\multirow{2}{*}{\diagbox{Method}{Scene}} & \multicolumn{3}{c}{cows} & \multicolumn{3}{c}{drift-turn} & \multicolumn{3}{c}{horsejump-high} & \multicolumn{3}{c}{kite-surf} & \multicolumn{3}{c}{mallard-water} & \multicolumn{3}{c}{mbike-trick} & \multicolumn{3}{c}{rhino} \\
\cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22}
 & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓  & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓ & PSNR↑ & SSIM↑ & Time↓\\
\midrule
Robust-Dyn~\cite{liu2023robust} & 24.6 & 0.684 & 890m  & 25.4  & 0.725 & 720m & 28.4 & 0.911 & 700m & 24.8 & 0.704 & 685m & 21.4 & 0.542 & 780m & 28.4 & 0.869 & 782m & 29.6 & 0.904 & 824m \\
NLA~\cite{kasten2021layered} & 25.9  & 0.783 & 317m & 25.3  & 0.723  & 308m & 28.2 & 0.867 & 324m & 28.7 & 0.776 & 295m & 22.2 & 0.600 & 328m & 31.0 & 0.885 & 294m & 30.0 & 0.873 & 293m\\
CoDeF~\cite{ouyang2023codef} & 26.5 & 0.801 & \graycell{28m}  & 26.9  & 0.818  & 32m & 30.1 & 0.904 & \graycell{28m} & 32.7 & 0.925 & 30m & 28.8 & 0.881 & \graycell{28m} & 32.3 & 0.914 & 28m & 29.6 & 0.878 & \graycell{28m} \\
\hline
3DGS~\cite{kerbl20233d}  & 25.8 & 0.895 & \redcell{12m} & 23.8 & 0.815 & \yellowcell{16m} & 22.7 & 0.854 & \yellowcell{14m} & 23.9 & 0.692 & \redcell{8m} & \multicolumn{3}{c}{N/A} & 23.7 & 0.870 & \redcell{10m} & 29.1 & 0.921 & \redcell{7m}  \\
Deform-3DGS~\cite{yang2023deformable3dgs} & 30.2 & 0.952 & 79m & 27.6 & 0.897 & 68m & 29.3 & 0.945 & 60m & 27.9 & 0.820 & 42m & \multicolumn{3}{c}{N/A} & 33.8 & 0.938  & 32m & 33.2 & 0.947 & 38m\\
\hline
\modelname (w/ \textit{3k} iterations) & \graycell{35.7} & \graycell{0.981} & \yellowcell{18m} & \graycell{36.2} & \graycell{0.979} & \redcell{12m} & \graycell{34.8} & \graycell{0.978} & \redcell{8m} & \graycell{39.5} & \graycell{0.979} & \yellowcell{9m} & \graycell{36.7} & \graycell{0.981} & \redcell{13m} & \graycell{42.4} & \graycell{0.989} & \yellowcell{12m} & \graycell{37.4} & \graycell{0.982} & \yellowcell{14m}\\
\modelname (w/ \textit{5k} iterations) & \yellowcell{39.8} & \yellowcell{0.991} & 39m & \yellowcell{39.3} & \yellowcell{0.985}  & \graycell{25m} & \yellowcell{38.4} & \yellowcell{0.985} & \yellowcell{14m} & \yellowcell{42.3} & \yellowcell{0.987} & \graycell{17m} & \yellowcell{40.1} & \yellowcell{0.990} & \yellowcell{26m} & \yellowcell{45.7} & \yellowcell{0.993} & \graycell{22m} & \yellowcell{42.4} & \yellowcell{0.992} & \graycell{28m} \\
\modelname (w/ \textit{10k} iterations) & \redcell{46.3} & \redcell{0.998} & 116m & \redcell{43.1}  & \redcell{0.991} & 65m & \redcell{43.7} & \redcell{0.992} & 34m & \redcell{47.0} & \redcell{0.995} & 43m & \redcell{45.3} & \redcell{0.996} & 65m & \redcell{48.7} & \redcell{0.995} & 48m & \redcell{47.2} & \redcell{0.997} & 73m\\

\bottomrule
\bottomrule

\end{tabular}
}
% \vspace{-2mm}
\caption{Quantitative results of Video Reconstruction on DAVIS. We present the results for PSNR, SSIM and training Time,
with each cell colored to indicate the \sethlcolor{lightred}\hl{best}, \sethlcolor{lightyellow}\hl{second best}, and \sethlcolor{lightgray}\hl{third best} performances (best viewed in color). N/A indicates the inability to reconstruct all frames within the video, as the conventional COLMAP algorithm, employed in both 3DGS and Deform-3DGS methodologies, encounters limitations in acquiring 3D points pertinent to every frame.
% All expkeriments are conducted with a single A100 GPU. 3k/5k/10k: 3k/5k/10k.
Our method \modelname is trained with different total numbers of iterations (3k, 5k, and 10k), attaining different accuracy-time trade-off.
↑: the higher, the better.
↓: the lower, the better.
% \jay{Add another figure to summarize the results (i.e., average over 28 videos for each method).}
% \inkyu{Do you mean the table containing the average number of them?}
% \jay{Let's do a table to summarize the average performance. I was also thinking about having a figure to show the performance for each video (eg, y-axis PSNR and x-axis video name).}
\inkyu{Make it curve, put this one into supple /
Add Nerv results}
}
\label{tab:recon_quan}
% \vspace{-2mm}
\end{table*}

==> table/recon_table_time.tex <==

% LPIPS↓ 
% CoDeF & \graycell{31.26} & 0.9254 & 0.0735 & 29.11 & 0.9451 & 0.0601 \\
% RobustDyn & 24.58 & 0.9520 & 0.0824 & 32.50 & 0.9713 & 0.0362 \\
% Ours & \redcell{41.54} & \redcell{0.9873} & \redcell{0.0234} & \redcell{42.63} & 0.9951 & \redcell{0.0052} \\
\begin{table}
\centering
\resizebox{0.99\linewidth}{!}{
\begin{tabular}{lccccccc}
\toprule
\multicolumn{8}{c}{Video metric: WarpSSIM↑} \\
\toprule
\toprule
% & \multicolumn{2}{c}{bear} & \multicolumn{2}{2}{car-shadow} & \multicolumn{2}{c}{dog} & \multicolumn{2}{c}{elephant} & \multicolumn{2}{c}{gold-fish} & \multicolumn{2}{c}{hike} & \multicolumn{2}{c}{horsejump-low} \\
Method  & bear & \multicolumn{1}{c}{car-shadow} & \multicolumn{1}{c}{dog} & \multicolumn{1}{c}{elephant} & \multicolumn{1}{c}{gold-fish} & \multicolumn{1}{c}{hike} & \multicolumn{1}{c}{horsejump-low} \\
% \cmidrule(lr){2-3} \cmidrule(lr){4-5} \cmidrule(lr){6-7} \cmidrule(lr){8-9} \cmidrule(lr){10-11} \cmidrule(lr){12-13} \cmidrule(lr){14-15}
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22}

\midrule
3D-GS &  &  &  &  &  &  \\
Deform-3D-GS &  &  &  &  &  &  \\
NLA &  &  &  &  &  & \\
CoDeF &  &  &  &  &  & \\
RobustDyn &  &  &  &  &  & \\
\hline
Ours (\textit{Fast}) &  &  &  &  &  & \\
Ours (\textit{Pro}) &  &  &  &  &  & \\
Ours (\textit{Ultra}) &  &  &  &  &  & \\
\bottomrule
\bottomrule
% & \multicolumn{2}{c}{lab-coat} & \multicolumn{2}{c}{longboard} & \multicolumn{2}{c}{motorbike} & \multicolumn{2}{c}{swing} & \multicolumn{2}{c}{blackswan} & \multicolumn{2}{c}{camel} & \multicolumn{2}{c}{car-turn} \\
Method  & \multicolumn{1}{c}{lab-coat} & \multicolumn{1}{c}{longboard} & \multicolumn{1}{c}{motorbike} & \multicolumn{1}{c}{swing} & \multicolumn{1}{c}{blackswan} & \multicolumn{1}{c}{camel} & \multicolumn{1}{c}{car-turn} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22}

\midrule
3D-GS &  &  &  &  &  &  \\
Deform-3D-GS &  &  &  &  &  &  \\
NLA &  &  &  &  &  & \\
CoDeF &  &  &  &  &  & \\
RobustDyn &  &  &  &  &  & \\
\hline
Ours (\textit{Fast}) &  &  &  &  &  & \\
Ours (\textit{Pro}) &  &  &  &  &  & \\
Ours (\textit{Ultra}) &  &  &  &  &  & \\

\bottomrule
\bottomrule
% & \multicolumn{2}{c}{flamingo} & \multicolumn{2}{c}{hockey} & \multicolumn{2}{c}{kid-football} & \multicolumn{2}{c}{lucia} & \multicolumn{2}{c}{scooter-gray} & \multicolumn{2}{c}{boat} & \multicolumn{2}{c}{car-roundabout} \\
Method  & \multicolumn{1}{c}{flamingo} & \multicolumn{1}{c}{hockey} & \multicolumn{1}{c}{kid-football} & \multicolumn{1}{c}{lucia} & \multicolumn{1}{c}{scooter-gray} & \multicolumn{1}{c}{boat} & \multicolumn{1}{c}{car-roundabout} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22}

\midrule
3D-GS &  &  &  &  &  &  \\
Deform-3D-GS &  &  &  &  &  &  \\
NLA &  &  &  &  &  & \\
CoDeF &  &  &  &  &  & \\
RobustDyn &  &  &  &  &  & \\
\hline
Ours (\textit{Fast}) &  &  &  &  &  & \\
Ours (\textit{Pro}) &  &  &  &  &  & \\
Ours (\textit{Ultra}) &  &  &  &  &  & \\

\bottomrule
\bottomrule
% & \multicolumn{2}{c}{cows} & \multicolumn{2}{c}{drift-turn} & \multicolumn{2}{c}{horsejump-high} & \multicolumn{2}{c}{kite-surf} & \multicolumn{2}{c}{mallard-water} & \multicolumn{2}{c}{mbike-trick} & \multicolumn{2}{c}{rhino} \\
Method  & \multicolumn{1}{c}{cows} & \multicolumn{1}{c}{drift-turn} & \multicolumn{1}{c}{horsejump-high} & \multicolumn{1}{c}{kite-surf} & \multicolumn{1}{c}{mallard-water} & \multicolumn{1}{c}{mbike-trick} & \multicolumn{1}{c}{rhino} \\
% \cmidrule(lr){2-4} \cmidrule(lr){5-7} \cmidrule(lr){8-10} \cmidrule(lr){11-13} \cmidrule(lr){14-16} \cmidrule(lr){17-19} \cmidrule(lr){20-22}

\midrule
3D-GS &  &  &  &  &  &  \\
Deform-3D-GS &  &  &  &  &  &  \\
NLA &  &  &  &  &  & \\
CoDeF &  &  &  &  &  & \\
RobustDyn &  &  &  &  &  & \\
\hline
Ours (\textit{Fast}) &  &  &  &  &  & \\
Ours (\textit{Pro}) &  &  &  &  &  & \\
Ours (\textit{Ultra}) &  &  &  &  &  & \\

\bottomrule
\bottomrule

\end{tabular}
}
\caption{Quantitative results (WarpSSIM) of Video Reconstruction on DAVIS.}
\label{tab:recon_warp}
\end{table}



==> table/tf_qual.tex <==
\begin{figure*}[!t]
    \centering 
    \includegraphics[width=0.9\textwidth]{icml2024/figures/tf_figure.pdf}
    \caption{\textbf{Qualitative results using TF Loss}}
    \label{fig:tf_figure}
    % \vspace{-3mm}
\end{figure*}
